CO emission survey of asymptotic giant branch stars with ultraviolet excesses

Context. The transition from the spherically symmetric envelopes around asymptotic giant branch (AGB) stars to the asymmetric morphologies observed in planetary nebulae is still not well understood, and the shaping mechanisms are a subject of debate. Even though binarity is widely accepted as a promising option. Recently, the presence of ultraviolet excesses in AGB stars has been suggested as a potential indicator of binarity. Aims. Our main goals are to characterise the properties of the circumstellar envelopes (CSEs) around candidate AGB binary stars, specifically those selected based on their UV excess emission, and to compare these properties with those derived from previous CO-based studies of AGB stars. Methods. We observed the 12CO ($J$=1-0) and 12CO ($J$=2-1) millimetre-wavelength emission in a sample of 29 AGB binary candidates with the IRAM-30 m antenna. We explored different trends between the envelope parameters deduced and compared them with those previously derived from larger samples of AGB stars found in the literature. Results. We derived the average excitation temperature and column density of the CO-emitting layers, which we used to estimate self-consistently the average mass-loss rate and the CO photodissociation radius of our targets. We find a correlation between CO intensity and IRAS 60${\mu}$m fluxes, revealing a CO-to-IRAS 60${\mu}$m ratio lower than for AGB stars and closer to that found for pre-planetary nebulae (pPNe). Conclusions. For the first time we have studied the mass-loss properties of UV-excess AGB binary candidates and estimated their main CSE parameters. The different relationships between 12CO and IRAS 60{\mu}m, with NUV and FUV are consistent with an intrinsic origin of NUV emission, but potential dominance of an extrinsic process (e.g. presence of a binary companion) in FUV emission.

==> tables/table2_pre.tex <==
\begin{table*}[t]

\renewcommand{\arraystretch}{1.3}
\small
\centering

\caption{Observational parameters of the sources.} 
\label{tab:sources}

\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}[b]

\begin{tabular}{l c c c c c c c}
\hline\hline 
Source & Variability$^{(a)}$   & Period$^{(a)}$   & Spectra$^{(b)}$  & Composition$^{(b)}$   & Luminosity$^{(c)}$ & E(B-V) (ISM)$^{(d)}$ & E(B-V) (CSM)$^{(e)}$\\ 
 &  (type) &  $(\mathrm{days})$ &  (type) &  (type) &  $(\mathrm{L_{\odot}})$ & (mag) & (mag)\\
\hline 

AT-DRA & LB     &       ----    &      M4III D ~    &   O  & $1820 \pm 160$  & 0.018 & \\

BC-CMI & SRB     &      34.13  &       M4/5III D   &    O & $640 \pm 50$  & 0.032 & \\

BD-CAM & LB   &  ----   & S3.5/2 B  &  O & $2350  \pm  160$ & 0.99 & \\

BY-BOO & LB     &   ----    &      M4.5III B     &  O & $1750 \pm 160$  & 0.0098 & \\

CG-UMA & LB   &         ----    &      M4IIIa D &   O & $1970 \pm 180$  & 0.038 & \\

DF-LEO & SRB     &      70        &    M4III C ~    &   O & $880 \pm 70$  & 0.046 & \\

EY-HYA &  SRA       &    182.7     &    M7 D        &    O & $6300 \pm 1500$  & 0.043 & 0.0087\\

FH-VIR & SRB      &     70    &        M6III C ~    &   O & $1300 \pm 140$  & 0.037 & \\

IN-HYA & SRB         &  65        &    M3/4III D    &   O & $1070 \pm 100$  & 0.028 & \\

OME-VIR & LB     &       ----   &       M4.5:III C &     O & $1540 \pm 120$  & 0.042 & \\

R-LMI & M       &      372.19    &    M6.5-9e B  & O & $3000 \pm 400$  & 0.015 & 0.010\\

R-UMA & M     &  301.62 & M5-8e B & O  &  $5000  \pm  500$ & 0.025 & 0.012\\

RR-ERI & SRB    &       97         &   M5III C      &   O & $3200 \pm 300$  & 0.048 & 0.0072\\

RR-UMI & SRB          & 43.3     &     M4.5III C    &   O  & $1080 \pm 70$  & 0.023 & \\

RT-CNC &  SRB     &      89.8 &         M5III C     &    O & $2800 \pm 300$  & 0.040 & 0.0062\\

RU-HER & M      &   484.83  &      M6-7e B       &  O & $19000 \pm 3000$  & 0.069 & 0.017\\

RW-BOO & SRB       &    209  &         M5III: D ~   &   O & $2000 \pm 200$  & 0.015 & 0.0063\\

RZ-UMA & SRB  &  115    & M8 D ~  &  O &  $4700  \pm  400$ & 0.039 & 0.0062\\

ST-UMA &  SRB      &     110 &          M4III C ~    &   O & $2300 \pm 200$  & 0.018 & \\

SV-PEG & SRB       &    144.6  &       M7 D ~       &   O & $6000 \pm 600$  & 0.17 & 0.017\\

T-DRA & M        &     421.62  &      C6,2e C       &  C & $7900 \pm 1500$  & 0.040 & 0.0088\\

TU-AND & M    &  316.8  & M6e B  &  O & $6100  \pm  600 $ & 0.039 &  \\

UY-LEO &  LB       &     ----   &       M7III: D ~  &    O & $2200 \pm 200$  & 0.023 & \\

V-ERI & SRC       &    97.0     &     M7+II: C      &  O & $5700 \pm 600$ & 0.040 & 0.0085\\

VY-UMA & LB   &  ----   & C-N5 B  & C  &  $5100  \pm  500$ & 0.016 & 0.0037\\

W-PEG & M           &  345.5        & M6.5-7.5e B   &  O & $4400 \pm 500$  &  0.086& 0.0093\\

Y-CRB & SRB      &     300       &    M8III: D ~    &  O & $4000 \pm 400$ & 0.012 & 0.012\\

Y-GEM & SRB     &      160      &     M8 D ~      &    O & $6800 \pm 600$  & 0.051 & \\

Z-CNC & SRB        &   95.4         & M6III C ~     &  O & $3500 \pm 400$ & 0.038 & 0.010\\

\hline
\end{tabular} 
\begin{tablenotes}
\item \textbf{Notes.} Column (1): name of the source, Col (2): variability type of the source, Col (3): expansion period of the source when the source has a stable period, Col (4): spectral type of the source, Col (5): composition of the source (O oxygen star or C carbon star), Col (6): bolometric luminosity of the source, Col (7): reddening produced by the interstellar medium, Col (8): reddening produced by the circumstellar medium when available.
\item[(a)] Variability classification and pulsation periods have been obtain from the GCVS.
\item[(b)] Spectra and composition classifications have been obtained from the SIMBAD astronomical database \citep{SIMBAD}.
\item[(c)] Luminosity values have been obtained from integration of the SEDs.
\item[(d)] Interstellar medium reddening has been obtained from \cite{Schlegel_1998}.
\item[(e)] Circumstellar medium reddening has been estimated by the column densities of table \ref{tab:parameters} (when available) and with typical values of $N_{tot}/A_{V}=1.8\cdot10^{21} mag^{-1}cm^{-2}$ and $R_{V}=3.1$.
\end{tablenotes}

\end{threeparttable}
\end{adjustbox}

\renewcommand{\arraystretch}{1.0}


\end{table*}

==> tables/table5_pre.tex <==

\begin{table*}[h!]

\renewcommand{\arraystretch}{1.3}
\centering

\caption{Fluxes used in this study.} 
\label{tab:fluxes}

\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}[b]

\begin{tabular}{l c c c c c c c c}
\hline\hline 
Source & IRAS $[\mathrm{12 \mu m}]$ & IRAS$[\mathrm{25 \mu m}]$ & IRAS$[\mathrm{60 \mu m}]$ & IRAS$[\mathrm{100 \mu m}]$ & Galex epoch & GALEX NUV & GALEX FUV  & X-ray$^{(a)}$\\  
       & $(\mathrm{Jy})$ & $(\mathrm{Jy})$ & $(\mathrm{Jy})$ &  $(\mathrm{Jy})$ & $(\mathrm{Jy})$ &  $(\mathrm{\mu Jy})$ & $(\mathrm{\mu Jy})$ &        \\  
\hline 
AT-DRA & $48.1\pm1.4$ & $13.1\pm0.5$ & $2.19\pm0.15 $ & $0.9\pm0.3 $ & 2011-07-25 & $2145\pm 8$ & & NO \\
 & & & & & 2004-06-26 & $2217 \pm17$ & $172 \pm9 $ &\\
 & & & & & 2004-06-26 & $2208 \pm16 $ & $181 \pm9$ &\\
BC-CMI & $23.4\pm0.9 $ & $6.6\pm0.4$ & $0.94\pm0.08 $ & $\leq 1.0 $ & 2006-01-01 & $1013 \pm16$ & $55 \pm5 $ & NO\\
BD-CAM & $41\pm 2$ & $10.8\pm0.5$ & $1.59\pm0.19$ & $\leq 2.03$ & 2005-12-28 & $5970 \pm 40$ & $2330\pm30$ & D$^{(a)}$\\
BY-BOO & $69 \pm 3 $ & $18.60\pm0.11 $ & $2.9\pm0.4 $ & $\leq 1.16$ & 2004-06-05  & $3240\pm 30$ & $215 \pm9 $ & NO\\
 & & & & & 2008-07-03 & $3040 \pm 9$ & $213 \pm 5$ & \\
CG-UMA & $40 \pm 2 $ & $10.9 \pm0.8 $ & $1.69 \pm0.17 $ & $\leq 1.00$ & 2004-01-18 & $1491 \pm 23$ & $108 \pm 9$ & ND\\
 & & & & & 2004-01-31 & $1505 \pm4 $ & &\\
DF-LEO & $10.7 \pm0.4$ & $2.8 \pm0.2 $ & $0.61 \pm0.07 $ & $\leq 1.0$ & 2007-02-23 & $673 \pm4 $ & $39.6 \pm1.7$ & NO\\
 & & & & & 2004-02-23 & $471 \pm10 $ & $32 \pm4 $\\
 & & & & & 2009-01-30 & $623 \pm11$ & $36 \pm 4$\\
EY-HYA & $102 \pm16$ & $50\pm 2$ & $8.0\pm0.7$ & $2.8\pm0.2 $ & 2007-02-19 & $133.6 \pm1.7$ & $95.0 \pm1.7 $ & D$^{(b)}$\\
 & & & & & 2006-02-20 & $88 \pm5 $ & $69 \pm 7$ &\\
FH-VIR & $18.8\pm 1.1 $ & $6.0\pm0.5 $ & $1.19\pm0.18 $ & $\leq 1.0$ & 2006-05-01 & $417 \pm 3$ & $44.8 \pm1.9$ & NO\\
 & & & & & 2004-04-14 & $426 \pm13 $ & $56\pm9 $ \\
 & & & & & 2004-04-14 & $366 \pm12$ & $45 \pm6$ \\
IN-HYA & $18.2\pm0.9$ & $5.2\pm0.4$ & $1.00\pm0.11$ & $\leq 1.0$ & 2006-02-23 & $580 \pm14$ & $44 \pm6 $ & ND\\
 & & & & & 2004-02-09 & $656 \pm4 $ & $43.4\pm1.9 $ & \\
OME-VIR & $62\pm 3 $ & $15.6\pm 1.2 $ & $2.8\pm0.3 $ & $\leq 1.2$ & 2004-0327 & $2950 \pm30$ & $179 \pm12 $ & NO\\
R-LMI & $430 \pm 50$ & $176 \pm 19 $ & $26 \pm 3 $ & $7.9 \pm 0.9$ & 2006-02-28 & $17 \pm2 $ & $\leq 5.75$ & ND\\
 & & & & & 2005-04-11 & $59.3 \pm1.1 $ & $2.4\pm0.7$ &\\
R-UMA & $94 \pm19$ & $55\pm 8$ & $7.0\pm0.8 $ & $2.8\pm0.2 $ & 2003-1208 & $59 \pm4 $ & $55 \pm 7$ & NO\\
 & & & & & 2006-01-06 & $117 \pm 2$ & $44.9 \pm1.9$ & \\
 & & & & & 2003-12-08 & $90 \pm8 $ & $59 \pm7 $ & \\
RR-ERI & $44 \pm 2$ & $20.4\pm 1.0 $ & $3.3 \pm0.3$ & $0.82\pm0.10 $ & 2007-10-20 & $485\pm10 $ & $28 \pm 4$ & ND\\
 & & & & & 2003-11-26 & $382 \pm3 $ & $27.1 \pm1.3 $\\
RR-UMI & $124\pm 4$ & $33.0\pm 1.3 $ & $5.2\pm0.5 $ & $1.12\pm0.15$ & 2005-03-07 & $6490 \pm 40$ & $1930\pm30$ & D$^{(b)}$\\
 & & & & & 2007-04-06 & $7830\pm60$ & $1810 \pm50$ & \\
RT-CNC & $73\pm 3$ & $29.1\pm 1.5 $ & $4.20\pm0.42$ & $1.40\pm0.11$ & 2006-02-20 & $206 \pm 7$ & $33 \pm 4$ & NO\\
 & & & & & 2009-01-03 & $173 \pm7$ & $40 \pm 6$ &\\
 & & & & & 2006-02-20 & $175 \pm11$ & $24 \pm7 $ &\\
RU-HER & $173\pm 19$ & $78 \pm 3$ & $11.4\pm0.9$ & $4.5\pm0.4$ & 2004-05-29 & $85 \pm3 $ & $\leq 5.75$ & ND\\
 & & & & & 2005-07-27 & $74.8\pm1.0 $ & $\leq 5.75$\\
RW-BOO & $61\pm3$ & $29.8\pm1.2$ & $5.6\pm0.5$ & $2.8\pm0.3 $ & 2007-04-08 & $369 \pm13 $ & $17\pm 5$ & NO\\
 & & & & & 2006-05-05 & $451 \pm2 $ & $29.5\pm1.6$\\
RZ-UMA & $46.5\pm1.9$ & $22.1\pm0.9$ & $4.0\pm0.4$ & $1.92\pm0.17$ & 2006-12-26 & $20 \pm 4$ & $8 \pm 4$ & ND\\
 & & & & & 2005-11-21 & $15.6 \pm0.9 $ & $\leq 5.75$ &\\
ST-UMA & $43.9\pm1.8$ & $18.8\pm0.9$ & $3.1\pm0.3$ & $1.11\pm0.12$ & 2004-03-08 & $994 \pm14$ & $168 \pm13$ & NO\\
SV-PEG & $265\pm 11$ & $146\pm9$ & $24\pm3$ & $9.9\pm1.0$ & 2006-09-20 &  $30 \pm 4$ & $\leq 5.75$ & NO \\
 & & & & & 2004-09-26 & $28.5 \pm0.7$ & $\leq 5.75$\\
T-DRA & $197\pm14 $ & $66 \pm 3$ & $15.8 \pm0.9$ & $5.7\pm0.3$ & 2005-06-20 & $\leq 5.75$ & $7.93\pm1.1$ & D$^{(b)}$\\
 & & & & & 2007-07-12 & $32 \pm3$ & $\leq 5.75$\\
TU-AND & $20.5\pm 1.2$ & $7.6\pm0.6$ & $1.23\pm0.14$ & $\leq 1.41$ & 2004-10-02 & $22.8 \pm1.3$ & $\leq 5.75$ & NO\\
 & & & & & 2003-10-07 & $8 \pm2$ & $\leq 5.75$ &\\
\hline
\end{tabular} 
\end{threeparttable}
\end{adjustbox}

\renewcommand{\arraystretch}{1.0}

\end{table*}


\begin{table*}[h!]

\renewcommand{\arraystretch}{1.3}
\centering


\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}[b]

\begin{tabular}{l c c c c c c c c}  
\hline 
UY-LEO & $8.6\pm0.3$ & $3.9\pm0.3$ & $0.6\pm0.06 $ & $\leq 1.0$ & 2005-03-16 & $132 \pm4 $ & $24 \pm5 $ & ND(*)\\
 & & & & & 2006-02-06 & $167 \pm2 $ & $30 \pm1.5$\\
V-ERI & $326\pm10$ & $184\pm 7$ & $24\pm2$ & $7.2\pm0.6 $ & 2005-11-03 & $142 \pm2 $ & $79 \pm 3$ & ND(*)\\
 & & & & & 2007-01-07 & $56 \pm5 $ & $54 \pm8 $ & \\
VY-UMA & $52\pm2$ & $14.0\pm0.7$ & $4.8\pm0.4$ & $4.9\pm0.4$ & 2004-01-21 & $93 \pm 7$ & $10\pm4 $ & ND\\
 & & & & & 2004-01-21 & $84 \pm6$ & $8 \pm3$ &\\
 & & & & & 2006-01-07 & $234 \pm3$ & $6.6\pm0.8 $ &\\
W-PEG & $218\pm9 $ & $94\pm4$ & $13.1\pm 1.2$ & $3.5\pm0.4$ & 2009-08-28 & $157.3 \pm1.7 $ &  & ND\\
 & & & & & 2006-10-02 & $201 \pm 7$ & $13 \pm3$\\
Y-CRB & $27.0\pm1.1$ & $10.8\pm0.5$ & $1.67\pm0.12$ & $0.62\pm0.09$ & 2005-07-28 & $9.2 \pm0.6 $ & $\leq 5.75$ & NO\\
 & & & & & 2004-05-15 & $15 \pm 4$ & $\leq 5.75$ & \\
Y-GEM & $28.5\pm 1.7$ & $9.0\pm0.6$ & $1.23\pm0.11$ & $\leq 1.0 $& 2006-01-04  & $11100\pm 50$ & $10560 \pm 90$ & D$^{(b)}$\\
 & & & & & 2008-12-28 & $3690 \pm20 $ & $2230 \pm 30$\\
 & & & & & 2008-01-19 & $1613 \pm 7$ & $1380 \pm10 $\\
Z-CNC & $44\pm 2$ & $22.0\pm1.3$ & $3.0\pm0.3$ & $1.34\pm0.15$ & 2008-02-24 & $73.5 \pm1.7$ & $13.7 \pm1.3 $ & ND(*)\\
 & & & & & 2008-01-28 & $72 \pm 5$ & $11 \pm 3$ & \\
\hline
\end{tabular} 
\begin{tablenotes}
\item \textbf{Notes.} Column (1): name of the source, col (2): IRAS $12\mu\, m$ flux, col (3): IRAS $25\mu\, m$ flux, col (4): IRAS $60\mu\, m$ flux, col (5): IRAS $100\mu\, m$ flux, col (6): GALEX epoch, col (7): GALEX NUV flux, col (8): GALEX FUV flux, col (9): SWIFT X-ray detections (D: detected, ND: non-detected, NO: non-observed), (*) indicates XMM-Newton observation available. (a) \cite{Lima_2022}, (b) \cite{Ortiz_2021}.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}

\renewcommand{\arraystretch}{1.0}

\end{table*}
